A Hybrid Framework Using a QUBO Solver For Permutation-Based Combinatorial Optimization

In this paper, we propose a hybrid framework to solve large-scale permutation-based combinatorial problems effectively using a high-performance quadratic unconstrained binary optimization (QUBO) solver. To do so, transformations are required to change a constrained optimization model to an unconstrained model that involves parameter tuning. We propose techniques to overcome the challenges in using a QUBO solver that typically comes with limited numbers of bits. First, to smooth the energy landscape, we reduce the magnitudes of the input without compromising optimality. We propose a machine learning approach to tune the parameters for good performance effectively. To handle possible infeasibility, we introduce a polynomial-time projection algorithm. Finally, to solve large-scale problems, we introduce a divide-and-conquer approach that calls the QUBO solver repeatedly on small sub-problems. We tested our approach on provably hard Euclidean Traveling Salesman (E-TSP) instances and Flow Shop Problem (FSP). Optimality gap that is less than $10\%$ and $11\%$ are obtained respectively compared to the best-known approach.

==> Equivalent_TSP_formulation.tex <==
\subsection{Data Perturbation} \label{perturbation}

One challenge with solving TSP is that there could be a large variant on the distance matrix, which is a disadvantage to a local search algorithm as the trajectory might be hindered by an energy landscape comprising local minima with great depths. Recall that the probability of acceptance of a simulated annealing based algorithm depends on the difference of the function value and the neighboring value and large differences result in small probability of acceptance. 

We use the result from Karp \textcolor{red}{include citation} where it is shown that we can change all the distance to or from a particular city by a constant and preserve the ranking of optimality of the solutions. Furthermore, to determine the distance to be perturbed for a particular city $i$, $\Delta_i$, we use the result from \textcolor{red}{citation} to minimize the variance of all the distances.

We need to decide on all such $\Delta_i$'s to change $d_{ij}$ to $d_{ij}+\Delta_i + \Delta_j$. We want to minimize the overall variance as a similar distance value intuitively helps a local search algorithm to find a solution quicker. The following lemma gives us a systematic way to minimize the variance of the distance data.

With the data perturbation trick, we illustrate that we are able to improve the performance of the solution of the DA on TSP instance in Figure \ref{improve}. 




==> Large_Scale_TSP.tex <==


We are interested in focusing on decomposing our problems into instances of a certain size, hence in the clustering stage, we use the constrained $k$-means clustering algorithm \cite{bradley2000constrained}. The benefit of this approach is that we have better control over the size of the clusters suitable for QS. 







==> Overcoming_Parameter_Tuning_in_TSP.tex <==
%\subsection{Parameter Tuning}

 
%The next challenge is to overcome the problem of parameter tuning to balance between the objective QUBO and the constraint QUBO. This issue is silent among the research community working on QUBO. In Figure \ref{improveeffect}, we show that by tuning the weight coefficient, we are able to get better solutions. 

After clustering, we use the variance-minimizing distance scaling to change the objective to make the objective landscape smoother.

%We then use our trained MLP to predict a good weight coefficient for each given instance. Note however that the MLP is trained specifically for smaller instances. For our experiments (reported below), we training our neural network with instances of 30 or less number of cities. 



%\begin{figure}[ht]
%\begin{center}
%\includegraphics[scale=0.3]{figs/graph.tex}
%\includegraphics[scale=0.2]{MLPpicture.png}
%\caption{MLP architecture} \label{fig:img1}
%\end{center}
%\end{figure}

%several approaches to tune the weight parameter for the TSP QUBO formulation. More specifically, we consider tree based Parzen Estimator, as well as a method we call the zooming method.


%\subsubsection{Multilayer Perceptron}

%By using the data that we obtained from the zooming method and hyperopt tuning method, we build the MLP. 


%The training data obtained from our zooming method, which comprises feasible solutions to TSP instances and the corresponding weight parameters, are used to build a neural network to train a regression model.  The motivation is so that when we are given a new TSP instance, the neural network will predict a suitable weight parameter that will work well on the QUBO solver to obtain a near optimal solution.


%Even though our goal is to predict the optimum constraint weight for the QUBO model, it turns out that it is easier to predict $\frac{\text{ Suitable weight}}{\text{Longest edge length}}$.
%We transform our data to a range between $0$ and $1$ and build a network comprising $362$ edge weights.

%The features used in the neural network are stated in Table \ref{nnfeatures}. The last 3 
%features are well-known graph features that can be derived from eigenvalues of the distance matrix and its laplacian.
%{\tiny
%\begin{table}
%\begin{center}\midsepremove
%\begin{tabular}{ll} 
%\midrule
%Feature Name & Derivation  \\ 
%\midrule
%Iteration Number & $log_{10}$(Number of QS iterations)\\
%Minimum Edge Weight & Min. $d_{ij} \forall{(i,j) \in E}$  \\
%Maximum Edge Weight & Max. $d_{ij} \forall{(i,j) \in E}$  \\
%Mean Edge Weight & $\sum_{(i,j) \in E} \frac{d_{ij}}{|E|}$ \\
%Median Edge Weight & $med(d_{ij}) \forall{(i,j) \in E}$ \\
%Edge Weight Variance & $\sigma_{d_{ij} \forall{(i,j) \in E}}^2$ \\
%Number of Vertices & $|V|, V \in G(V,E)$ \\
%Number of Edges & $|E|, E \in G(V,E)$ \\
%\midrule
%Greedy heuristic & nearest neighbor \\
%Two-opt heuristic & local search\\
%\midrule
%Min. Spanning Tree & Kruskal's algorithm \\
%\midrule
%Spectral Radius & $\rho(G)$ \\
%Condition Number & $\kappa(G)$\\%$\frac{\rho(G)}{eigenvalue_{min}(G)}$ \\
%\midrule
%Algebraic Connectivity  & $\Lambda(G)$\\
%\bottomrule
%\end{tabular}
%\caption{Features and Derivation}\label{nnfeatures}
%\end{center}\midsepdefault
%\end{table}
%}

==> Projection_to_the_Closest_Feasible_Solution.tex <==
\section{Projection to the Closest Feasible Solution}

With suitable weight parameter and perturbed distances, we find that DA performs better. However, we still find that it is possible to get an infeasible solution. We might end up with an infeasible solution because the solver is along the trajectory to a better solution but it hasn't attain it yet. %Note that DA solver is a black box solver doesn't disclose what is happening in the intermediate step and the termination condition is the number of iterations used.

If such a scenario happens, we consider projection of our current infeasible solution to a feasible solution. Recall that for our TSP formulation, we are using a $2$-indexed formulation, where the first index is the city index and the second index is the slot index. If we represent the feasible solution as a matrix, a feasible solution is a permutation matrix. 

In terms of Hamming distance, we find that the problem of finding the closest permutation matrix to be a linear programming problem. Suppose we have obtain $y_{i,u}, i,u\in \{1, \ldots , n\}$ a solution which is binary but not feasible. To obtain $x_{i,u}$ that is feasible, their Hamming distance can be written as \begin{equation}(x_{i,u}-y_{i,u})^2=x_{i,u}^2-2x_{i,u}y_{i,u}+y_{i,u}^2=(1-2y_{i,u})x_{i,u}+y_{i,u} \end{equation}

Hence, to solve the projection problem, we just have to solve the following binary linear programming problem.

\begin{equation}\min_x (1-2y_{i,u})x_{i,u} \end{equation}

subject to \begin{equation}\sum_{u=1}^n x_{i,u}=1, \forall i \in \{1, \ldots, n\}\end{equation}

\begin{equation}\sum_{i=1}^n x_{i,u}=1, \forall u \in \{1, \ldots, n\}\end{equation}

which is just an assignment problem which can be solved in polynomial time.  
%\section{Moving Away from a Particular Solution}


==> QUBO_formulation_for_TSP.tex <==
\section{Application 1: Traveling Salesman Problem (TSP)}

A popular formulation of TSP is the  Dantzig-Fulkerson-Johnson (DFJ) formulation \cite{dantzig1954solution} which involves exponentially many equations to impose subtour elimination.
The standard approach for solving this formulation involves using techniques such as cutting plane methods. The conversion from this MIP to the corresponding QUBO would not be scalable as that would introduce exponentially many terms in the objective function. Alternatively, the Miller-Tucker-Zemlin (MTZ) formulation \cite{miller1991integer} involves only quadratic number of constraints. However, such formulation would still involve slack variables and hence not suitable to directly transfer to a QUBO model. 

In \cite{lucas2014ising}, a QUBO formulation that only involves a quadratic number of terms in the number of cities is proposed. Without loss of generality, we can focus on the case where the graph is fully connected, as we can always introduce edges of infinite distances otherwise. We let $d_{uv}$ be the distance between city $u$ and city $v$. We require $n^2$ variables for an $n$-city instance. The first subscript of $x$ represents the city and the second indicates the order that the city is going to be visited at. That is $x_{v,j}$ is the indicator variable that the city $v$ is the $j$-th city to be visited. Notice that the constraint implies that this satisfies the permutation condition.

The formulation is as follows:

\begin{equation*}\min_{x} H_B(x) + AH_A(x) \end{equation*}

Here \begin{equation*}H_B(x)=\sum_{(u,v) \in E} d_{uv} \sum_{j=1}^n x_{u,j}x_{v,j+1}\end{equation*} describes the total distance travelled and 

\begin{equation*}H_A = \sum_{v=1}^n \left( 1-\sum_{j=1}^n x_{v,j}\right)^2 + \sum_{j=1}^n \left( 1-\sum_{v=1}^n x_{v,j}\right)^2 \end{equation*} describes the constraints to be a feasible cycle.




%\cite{lucas2014ising} states that if $A$ is bigger than the maximum magnitude of the distance, then the QUBO formulation is indeed equivalent to the original TSP instance, however, though the problems are equivalent mathematically, when it comes to local search algorithm such as Digital Annealer, their performance differs. 



==> stitchingtsp.tex <==
%\subsection{Stitching Algorithm} 


Let $k$ be the number of clusters and largest cluster size  be $|V_c|$. The stitching algorithm is outlined as follows: 

\begin{enumerate}
\item  We define the least cost flip value $\Delta_{ij}$ between all cluster pairs to be the least cost of performing 2-opt to stitch the two clusters $i$ and $j$ together. The time complexity is  $ O(k^2{|E_c|}^2)$.
\item To determine the ordering of stitching clusters, we solve a minimum cost Hamiltonian path problem by reusing our QUBO TSP model presented above (except it seeks a minimum Hamiltonian path instead of cycle) with $\Delta_{ij}$ on the edges. 
%We reuse DA with Hamiltonian path formulation for this.
\item Finally, we construct the final solution for the original problem by stitching adjacent clusters derived from Step 2 via 2-opt. The stitching scheme is illustrated in Figure \ref{stitch}.
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=8cm]{stitchingSchemeNew.eps}
\caption{Stitching procedure}\label{stitch}
\end{center}
\end{figure}

\end{enumerate}

As the last local improvement step, we perform a standard $2$-opt operation on the overall solution.




%\textcolor{red}{An alternative stitching procedure that we adopt is we randomly switch the order of stitching. We report the best of the two versions of the stitching procedure in our numerical simulation. }



%\textcolor{red}{more details on stitching to be added}

%add figure?
